Survey on Reliable Deep Learning-Based Person Re-Identification Models: Are We There Yet?

Intelligent video-surveillance (IVS) is currently an active research field in computer vision and machine learning and provides useful tools for surveillance operators and forensic video investigators. Person re-identification (PReID) is one of the most critical problems in IVS, and it consists of recognizing whether or not an individual has already been observed over a camera in a network. Solutions to PReID have myriad applications including retrieval of video-sequences showing an individual of interest or even pedestrian tracking over multiple camera views. Different techniques have been proposed to increase the performance of PReID in the literature, and more recently researchers utilized deep neural networks (DNNs) given their compelling performance on similar vision problems and fast execution at test time. Given the importance and wide range of applications of re-identification solutions, our objective herein is to discuss the work carried out in the area and come up with a survey of state-of-the-art DNN models being used for this task. We present descriptions of each model along with their evaluation on a set of benchmark datasets. Finally, we show a detailed comparison among these models, which are followed by some discussions on their limitations that can work as guidelines for future research.

==> Parts/Biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{BahramLavi.png}}]{Bahram Lavi}
recieved his Ph.D. degree in Computer Engineering from University of Cagliari (UNICA), Italy (2018). He is currently a Post-Doctoral Researcher with the University of Campinas (UNICAMP) at Institute of Computing (IC), where he conducts his research in the research group RECOD (Reasoning for Complex Data) on modeling an approach for \textit{Feature-space-time coherence with heterogeneous data}. 
His research interests include pattern recognition, computer vision, and machine learning with applications to forensic and intelligence video surveillance systems.
\end{IEEEbiography}

% if you will not have a photo at all:
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{ihsanPic.png}}]{Ihsan Ullah}
is working as a Senior Post-Doctoral Researcher in Data Mining & Machine Learning Group, Discipline of IT, College of Engineering \& Informatics, National University of Ireland Galway. He is also the Project Manager for H2020 project called ROCSAFE. 
He did his PhD from University of Milan. His area of research is designing deep neural network architectures with focus on imposing pyramidal structures. He is a reviewer of a number of high impact journals. He worked on several projects with collaborators such as IBM, Insight Center for Data Analytics Galway, and CVGL Stanford University. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mehdi_fatan.jpeg}}]{Mehdi Fatan}
received the M.Sc. degree in Mechatronic engineering from Azad University of Ghazvin, in 2012. Currently, he is a Ph.D. candidate at Department of Computer Engineering and Mathematics of Security, University Rovira i Virgili, Tarragona, Spain.
His research focuses on the areas of image and video analysis, computer vision, and machine learning.\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{anderson-photo.png}}]{Anderson Rocha}
is an associate professor at the Institute of Computing,
University of Campinas (Unicamp), Brazil, since 2009. His main interests include Digital Forensics, Reasoning for Complex Data and Machine Intelligence. He has been an associate editor of important international journals such as the IEEE Transactions on Information Forensics and Security (T.IFS), Elsevier Journal of Visual Communication and Image Representation (JVCI), the EURASIP/Springer Journal on Image and Video Processing (JIVP) and the IEEE Security & Privacy Magazine. He is an elected affiliate member of the Brazilian Academy of Sciences (ABC) and the Brazilian Academy of Forensic Sciences (ABC). He is a two-term elected member of the IEEE Information Forensics and Security Technical Committee (IFS-TC) and, currently, its chair for the 2019/2020 term. He is a Microsoft Research  and a Google Research Faculty Fellow, important academic recognitions given to researchers by Microsoft Research and Google, respectively. In addition, in 2016, he has been awarded the Tan Chin Tuan (TCT) Fellowship, a recognition promoted by the Tan Chin Tuan Foundation in Singapore. He has been the principal investigator of a number of research projects in partnership with public funding agencies in Brazil and abroad as well as national and multi-national companies having already deposited and licensed several patents. Since March 2019, he has been the Director of the Institute of Computing, University of Campinas (Unicamp).
\end{IEEEbiography}

\vfill
